Global analysis of regulatory network dynamics: equilibria and saddle-node bifurcations

In this paper we describe a combined combinatorial/numerical approach to studying equilibria and bifurcations in network models arising in Systems Biology. ODE models of the dynamics suffer from high dimensional parameters which presents a significant obstruction to studying the global dynamics via numerical methods. The main point of this paper is to demonstrate that adapting and combining classical techniques with recently developed combinatorial methods provides a richer picture of the global dynamics despite the high parameter dimension. Given a network topology describing state variables which regulate one another via monotone and bounded functions, we first use the {\em Dynamic Signatures Generated by Regulatory Networks} (DSGRN) software to obtain a combinatorial summary of the dynamics. This summary is coarse but global and we use this information as a first pass to identify ``interesting'' subsets of parameters in which to focus. We construct an associated ODE model with high parameter dimension using our {\em Network Dynamics Modeling and Analysis} (NDMA) Python library. We introduce algorithms for efficiently investigating the dynamics in these ODE models restricted to these parameter subsets. Finally, we perform a statistical validation of the method and several interesting dynamical applications including finding saddle-node bifurcations in a $54$ parameter model.

==> applications.tex <==
\subsection{Multiple saddle-node bifurcations, hysteresis, and isolas}
\label{sec:hysteresis and isolas}

Despite the remarkable accuracy of DSGRN predictions demonstrated in Section \ref{sec:saddlenode_TS}, there exist relatively small sub-regions of parameters for which there is evidence of richer dynamics than predicted. This occurs even in simple examples such as the Toggle Switch and in this section we demonstrate our ability to find such instances and explore some of the dynamics exhibited in these instances. 

In Section \ref{sec:saddlenode_TS} our numerical analysis hints to the fact that there is a strong correlation between parameter regions and saddle node behaviour, in particular one of these two possibilities is likely to hold:
\begin{itemize}
    \item $\pi_{\Xi^*}(\xi^*) \in R^*(5)$, then along the path \textbf{r} there exists a saddle-node bifurcation for some $d\in (1,\infty)$.
    \item $\pi_{\Xi^*}(\xi^*) \notin R^*(5)$, then for all $d\in[1,\infty)$ along \textbf{r} there exists a unique equilibrium.
\end{itemize}
This second element is also supported by the following intuition. For $d > 2$ both Hill functions are sigmoidal with $d$ controlling the incline of the steepest part of the sigmoid. Therefore, for the Toggle Switch with identified Hill coefficients, it seems reasonable to guess that the nullclines of $f^*$ move ``toward each other'' monotonically as $d \to \infty$. This intuition is shown in Figure \ref{fig:nullclines} and suggests that $f^*$ may undergo at most one saddle-node bifurcation with respect to $d$. 


\begin{figure}[t]
	\begin{center}
		\includegraphics[width = \textwidth, keepaspectratio=true, trim={0 0 0 1.2cm},clip]{nullclines.png}
		\caption{Toggle Switch nullclines for a parameter in $R^*(5)$ with Hill exponent varying through a saddle-node bifurcation. As both Hill functions become steeper, the nullclines tend to be closer to one another until the saddle-node bifurcation, at which point the nullclines intersect tangentially. Further increasing $d$ increases the area bounded between the nullclines and the three equilibria appear to move further apart from each other. 
		}
		\label{fig:nullclines}
\end{center}
\end{figure}
However, the techniques described in this paper provide the means to efficiently test this conjecture. Despite the fact that the parameter space is ``high'' dimensional, the combinatorial analysis suggests that if a counterexample exists, one might look for it near the boundary of $R^*(5)$. Then, using the efficient numerical methods described in this work, we easily find parameters which numerically demonstrate multiple bifurcations and surprisingly this conjecture appears to be false. 
Indeed, the numerical investigation suggests that parameters outside of $R^*(5)$ may undergo (at least) two saddle-node bifurcations along a Hill path at some Hill coefficients $1 < d_1 < d_2 < \infty$. For Hill coefficients in $[1, d_1)$ and $(d_2, \infty)$, the system is monostable and it is bistable in $(d_1 , d_2)$. This behavior is shown for two parameters in Figure \ref{fig:numerical_isolas}. 
Moreover, the transition between monostability and bistability need not be hysteretic with respect to the Hill coefficient.
Indeed, pairs of saddle-node bifurcations occurring along a single Hill path may be hysteretic (i.e.~connected by a single equilibrium branch) or form isolas which are disconnected from a ``main'' branch associated to stable equilibrium which persists for all Hill coefficients. The combination of these dynamic behaviors in this model suggests one possible cause for failures in the construction of synthetic biological switches. 
\if false
This means that, for any parameter outside $R(5)$ for which we were able to find one saddle node, we should be able to find a second one, where the two additional branches of equilibria disappear.
Considering the equilibrium branches involved in these two saddle node bifurcations, the two possible behaviour of the equilibria are either to be hysteretic, or to define an isola. The graphical difference between the two behaviours can be seen in the Figure \ref{fig:isolas}.

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = 0.7\textwidth, trim= 1.5cm 14cm 4.25cm 1.7cm, clip]{sketch_isolas}
		\caption{On the left, expected behavior of a saddle-node in the center region $\mathcal{R}$. On the right, an isola,  expected behavior of equilibria when a saddle-node is detected outside the center region. Vertical axes in this case is $\hill$, while the saddle-nodes are indicated by a red diamond. Unstable equilibria are drawn as dotted lines.}
		\label{fig:isolas}
	\end{center}
\end{figure}
To the best of our knowledge, only hysteretic behaviour is expected to be found in the toggle switch \cite{kuznetsov2004synchrony}, but we were able to identify parameters showcasing both behaviours.
\fi 
In Figure \ref{fig:numerical_isolas}, we present a plot of the Hill coordinate with respect to the $x_1$ coordinate of numerically found equilibria for two  different parameters outside of the center region. We can see how they differ in the fact that, in the first parameter, a continuous function can be plotted, while in the second one, the Hill coefficient is not a function of $x_1$ and creates an isola. In both cases, the saddles have been first found numerically, using the method presented in Section \ref{sec:equilibria}, then the equilibria have been numerically continued to produce the figures.

\begin{figure}[th]
	\begin{center}
		\includegraphics[width = 0.45\textwidth]{figure_hysteresis.png}
		\includegraphics[width = 0.45\textwidth]{figure_isolas.png}
		\caption{
			Branches of equilibria computed for the reduced Toggle Switch for varying $d$ via pseudo-arc length continuation depicting the two mechanisms which cause multiple saddle-node bifurcations. (Left) Hysteretic behaviour for the Toggle Switch found at parameter value $\lambda^*=[0.9243, 0.0506, 0.8125, 0.0779, 0.8161] $. (Right) An isola is found at $\lambda^* = [0.6470, 0.3279, 0.9445, 0.5301, 0.3908]$ indicating that multiple saddle-node bifurcations are possible without hysteretic switching.}
		\label{fig:numerical_isolas}
	\end{center}
\end{figure}

\subsection{Degenerate saddle-node bifurcations}
\label{sec:degenerate saddle-node bifurcations}
%\include{ts_regions_table}
In this section we numerically investigate and compare the saddle-node bifurcations in the Toggle Switch occurring near the ``corners'' of $R(5)$. We note how the description of the attractors given by DSGRN includes not only a count of the stable equilibria but also their relative position in a simplified phase space. This richer information can be used to further investigate the dynamical behaviour supported by a system by applying our combined combinatorial-numerical approach. 

Consider the simplest situation that all of the attractors in the Morse decomposition identified for each region of the combinatorial parameter space in Table \ref{tab:parameter_regions} is associated with a single stable equilibrium for some smooth vector field $f : (0, \infty)^2 \to \rr^2$ located in the indicated quadrant of the state space. We consider first a path through the continuous parameter space which visits the parameter regions in the order $R(5) \mapsto R(8) \mapsto R(7) \mapsto R(4) \mapsto R(5)$. In the combinatorial system, a continuous branch of equilibria can not cross the hyperplanes defined by the equations $x_1 = \gamma_1 \theta_{2,1}$ and $x_2 = \gamma_2 \theta_{1,2}$. Therefore, if $f$ is a faithful continuous representation of the combinatorial dynamics then the most parsimonious explanation for the sequence of Morse decompositions along this path is as follows. 

For parameters in $R(5)$, $f$ has (at least) one unstable equilibrium. When passing between regions $R(5)$ and $R(8)$, this unstable equilibrium and the stable equilibrium in $(1,0)$ disappear in a saddle-node bifurcation. Similarly, when passing between regions $R(5)$ and $R(4)$ this unstable equilibrium and the stable equilibrium in $(0,1)$ disappear in a saddle-node bifurcation. Therefore, along the boundary separating $R(4)$ and $R(7)$ these two saddle-node bifurcations collide in a codimension-2 cusp bifurcation and similarly on the boundary between $R(8)$ and $R(7)$. An analogous analysis of a path visiting the regions (in order) $R(5) \mapsto R(2) \mapsto R(3) \mapsto R(6 )\mapsto R(5)$ suggests another cusp bifurcation at the ``corner'' shared by $R(5)$ and $R(3)$. 

To contrast this behavior, consider a path visiting the parameter regions $R(5) \mapsto R(8) \mapsto R(9) \mapsto R(6) \mapsto R(5)$. For all regions along this path, the unique stable equilibrium is located in quadrant $(0,1)$ which is most likely modelled by the existence of a common smooth branch of equilibria which remains in this quadrant throughout the path. On the boundary between $R(5)$ and $R(6)$, the unstable equilibrium and the stable equilibrium in $(1,0)$ disappear in a saddle-node bifurcation much like on the boundary between $R(5)$ and $R(8)$. 
A similar situation occurs for paths visiting regions $R(5) \mapsto R(2) \mapsto R(1) \mapsto R(4) \mapsto R(5)$. This behaviour is not likely compatible with a cusp bifurcation at the "corner" between $R(5)$ and $R(1)$ or $R(9)$. Thus, our conjecture is that bifurcations for parameters at the ``corners'' shared by region $R(5)$ and regions $R(1), R(9)$ and those at the corners shared by $R(5)$ and regions $R(3), R(7)$ are caused by very different mechanisms. 


To investigate our conjecture, suppose once again that $f^*$ is the nondimensionalized Toggle Switch Hill model defined in section \ref{sec:reducing the number} with $6$ dimensionless parameters. For visualisation purposes, we  define a suitable dimension reduction map from from $\Lambda^*$ onto the rectangle $[0, 3]^2 \subset \rr^2$ which preserves these $9$ DSGRN parameter regions and the relative distances between parameters and the region boundaries. 

To start, suppose $\xi^* \in \Xi^*$ and define the related parameters $\setof*{a_1, b_1, a_2, b_2}$ by the formulas
\[
a_1 := \ell^*_{1,2} \qquad b_1 := \ell_{1,2}^* + \delta_{1,2}^* \qquad a_2 := \frac{\ell_{2,1}^*}{\gamma_2^*} \qquad b_2 := \frac{\ell_{2,1}^* + \delta_{2,1}^*}{\gamma_2^*}.
\]
Observe that if the reduced polynomial inequalities in Table \ref{tab:parameter_regions} are expressed in terms of these new parameters, then the $9$ DSGRN parameter regions as well as their boundaries are defined by linear manifolds. For example, region $R(5)$ is given by
\[
R(5) = \setof*{(a, b) \in \rr^2 \times \rr^2 : 0 < a_1 < 1 < b_1 \ \text{and} \ 0 < a_2 < 1 < b_2 }
\]
and the boundary separating $R(5)$ and $R(6)$ is given by 
\[
\partial R(5) \cap \partial R(6) = \setof*{(a, b) \in \rr^2 \times \rr^2 : 0 < a_1 < 1 < b_1, \ a_2 = 1, \ \text{and} \ 1 < b_2 }.
\]
Implicitly this defines a nonlinear transformation $\psi : \Xi^* \to \rr^2 \times \rr^2$ given by the formula $\psi(\xi^*) = (a, b)$ which maps each DSGRN region to a unique hyperplane in $\rr^2 \times \rr^2$.  

To complete the construction, fix positive constants $\overbar{a}_1, \overbar{a}_2>1$ and define another map $g : \rr^2 \times \rr^2$ by the formulas
\begin{equation}\label{eq:2dmap}
    g_1(a,b) = 
\begin{cases}
	b_2 & \text{if} \ b_2 \leq 1 \\
	1+\frac{ 1 - a_2}{b_2 - a_2} & \text{if} \  a_2 < 1 < b_2 \\
	2 + \frac{a_2-1}{\overbar{a}_2 - 1} & \text{if} \ 1 \leq a_2 
\end{cases}
\qquad 
g_2(a,b) = 
\begin{cases}
	b_1 & \text{if} \ b_1 \leq 1 \\
	1+\frac{ 1 - a_1}{b_1 - a_1} & \text{if} \ a_1 < 1 < b_1 \\
	2 + \frac{a_1-1}{\overbar{a}_1 - 1} & \text{if} \ 1 \leq a_1
\end{cases}
\end{equation}
Observe that the bounded subset $K_{\overbar{a}_1, \overbar{a}_2} \subset \image \psi$ defined by the formula
\[
K_{\overbar{a}_1, \overbar{a}_2} := \setof*{(a, b) \in \image \psi : \abs{a_i} \leq \overbar{a}_i, 1< \overbar{a}_i,  i = 1,2}.
\]
satisfies $g\left(K_{\overbar{a}_1, \overbar{a}_2}\right) \subset [0,3]^2$. 



We use the previous constructions to visualize the relative position of parameters as follows. Given a fixed collection of parameters $\setof*{\xi^*_1, \dotsc, \xi^*_M} \subset \Xi^*$ we choose $\overbar{a}_1, \overbar{a}_2$ sufficiently large so that $\psi(\xi^*_j) \in K_{\overbar{a}_1, \overbar{a}_2}$ for $1 \leq j \leq M$. Therefore, the mapping $g \circ \psi : \Xi^* \to [0,3]^2$ satisfies the following properties. 
\begin{enumerate}
\item Each of the $9$ parameter regions is mapped to a distinct unit square in $[0,3]^2$ and their relative positions are preserved. In fact, $g \circ \psi$ has been constructed so that the images of these regions are simply obtained by superimposing the graph in Figure \ref{fig:TS}(b) onto $[0, 3]^2$. We let $S(i) := g \circ \psi (R^*(i))$ denote these unit squares for $1 \leq i \leq 9$. 
\item Each boundary separating a pair of parameter regions is mapped into a line of the form $g_i = j$ with  $i \in \setof*{1,2}$ and $j \in \setof*{1,2,3}$. In other words, boundaries of parameter regions are mapped onto boundaries of the corresponding unit square and relative positions of the boundaries are also preserved. 
\item Relative proximity to boundaries is preserved. Specifically, suppose $\xi_1, \xi_2 \in R^*(j)$ and $\operatorname{dist}(\xi_1, \partial R(j)) < \operatorname{dist}(\xi_2, \partial R(j))$, then $\operatorname{dist}(g \circ \psi ( \xi_1), \partial S(j))  < \operatorname{dist}(g \circ \psi ( \xi_2), \partial S(j))$.
\end{enumerate}
Given this projection of the parameter space into a two-dimensional Euclidean space we now visually investigate the behavior of saddle-node bifurcations along the boundary of $R^*(5)$. 

For each parameter sample $\lambda \in \Xi^*$, we are interested in finding any saddle node bifurcation that happens along the path $\curve(s)$ as presented in Section \ref{sec:equilibria}.

The first visual result we present is an overview of parameters that undergo saddle nodes at different Hill coefficients. For this, we find saddle nodes with respect to the Hill coefficient, then project the parameter over the $[0,3]^2$ square and represent the Hill coefficient as a heat map.
In Figure \ref{fig:heat_map}, on the left the projection \eqref{eq:2dmap} is used, while the color indicates the lowest Hill coefficient $d$ for which we could find a saddle node at the given parameter value. On the right Figure, there is a scatter plot of all parameters considered. 
These includes information on parameters that never undergo a saddle node, but also on parameters that undergo more than one saddle node, such as discussed in Section \ref{sec:hysteresis and isolas}. 

\begin{figure}
\begin{center}
\includegraphics[width = 0.475\textwidth%, trim = 1cm 0 0 4.9cm, clip
]{dsgrn_heat_plot.pdf}
\includegraphics[width = 0.475\textwidth%, trim = 1cm 0 0 4.9cm, clip
]{all_results.pdf}
\caption{Left: Using the projection presented in Equation \ref{eq:2dmap}, a heat map is plotted, indicating the smallest Hill coefficient undergoing a saddle node. Right: Using the same projection, parameters are plotted in blue if they don't undergo any saddle node, in green if they undergo a single saddle node, in orange if they undergo multiple saddle nodes and in red if the bisection algorithm found a saddle node that was not numerically confirmed with Equation \eqref{eq:num_saddle_node}}
\label{fig:heat_map}
\end{center}
\end{figure}

At first glance, Figure \ref{fig:heat_map} further supports the idea that choosing parameters in $R^*(5)$ has the highest likelihood of giving us a saddle node for relatively low Hill coefficient. 

Looking at this map, we observe that the bottom left of the center region seems to be the best location for a practical bistable switch, since most parameters in that section undergo a saddle node at low Hill coefficient, and thus support bistability for most large Hill coefficients. We notice how there are saddle nodes taking place outside the center region, but most of them undergo two saddle nodes, thus for high enough Hill coefficient they again present a unique stable fixed point, as discussed in Section \ref{sec:hysteresis and isolas}.

Crucially, this plot supports the claim that saddle-node bifurcations disappear into a cusp (or other codimension-2) bifurcation along a loop around the points $(1,1)$ or $(2,2)$. However, along a loop around $(1,2)$ or $(2,1)$, saddle-node bifurcations seem to disappear ``at infinity''. This is consistent with the observations we obtained from only the combinatorial dynamics using DSGRN, and that we presented at the beginning of this Section.
 

While the presented description encompasses the majority of the parameter values, there are still some outliers.
Indeed, we are able to find a handful of parameters in $R^*(3)$ that undergo two bifurcations. These parameters are close to the corner with $R^*(5)$ and can be seen in Figure \ref{fig:heat_map}.
These results underline that even for simple nonlinear systems there is sufficient complexity that any simple broadly sweeping overview will have points of failure. 
Nonetheless this paper presents methods to look at the general behaviour of systems, giving significant support to Figure \ref{fig:strategy}.
Let us remind the reader that each ``corner'' considered in Figure \ref{fig:heat_map} corresponds to a 4-dimensional surface in the full parameter space.
